Inverse Optimal Control as an Errors-in-Variables Problem

Inverse optimal control (IOC) is about estimating an unknown objective of interest given its optimal control sequence. However, truly optimal demonstrations are often difficult to obtain, e.g., due to human errors or inaccurate measurements. This paper presents an IOC framework for objective estimation from multiple sub-optimal demonstrations in constrained environments. It builds upon the Karush-Kuhn-Tucker optimality conditions, and addresses the Errors-In-Variables problem that emerges from the use of sub-optimal data. The approach presented is applied to various systems in simulation, and consistency guarantees are provided for linear systems with zero mean additive noise, polytopic constraints, and objectives with quadratic features.

==> bayesianet.tex <==
\begin{tikzpicture}[->,>=stealth',shorten >=0.pt,auto,node distance=1.4cm,>=stealth',bend angle=45,auto]
\tikzstyle{place}=[circle,very thick,draw=black!75,fill=blue!20,minimum width=1cm]
\tikzstyle{placel}=[ellipse,very thick,draw=black!75,fill=blue!20]
\tikzstyle{red place}=[place,fill=red!20]
\tikzstyle{green place}=[place,fill=yellow!20]
\tikzstyle{transition}=[rectangle,very thick,draw=green!75,fill=blue!20,minimum size=2mm]
\tikzstyle{every label}=[red]

\begin{scope}[scale=0.8,transform shape]

\node [red place] (beta) {$\beta$};

\node [green place] (Yd) [right of=beta] {$\{Y_d\}_{d=1}^D$};

\node [red place] (U) [right of = Yd] {$U$};

\node [green place] (Ud) [right of = U] {$\{U_d \}_{d=1}^D$};

\node [red place] (SigmaU) [right of = Ud] {$\Sigma_U$};





\path (beta) edge node {} (Yd);
\path (U) edge node {} (Yd);
\path(U) edge node {} (Ud);
\path(SigmaU) edge node {} (Ud);


\end{scope}
\end{tikzpicture}

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
